A Linear Kernel for Planar Semitotal Domination

A set of vertices $S$ in a graph $G$ is a semitotal dominating set if $S$ is a dominating set and every vertex in $S$ has a witness, that is, another vertex in $S$ within distance at most two. The Semitotal Domination problem asks whether $G$ admits such a set of size at most $k$. We study this problem parameterized by the solution size. We provide a linear kernel of size $358k$ on planar graphs, a result that adds to several existing linear kernels for other domination variants on planar graphs. Additionally, we show Semitotal Domination is $W[2]$-hard on split graphs, on bipartite graphs and on $t$-claw-free graphs, it is $W[1]$-hard on circle graphs.

==> conf/lipic-fixes.tex <==

\setcounter{secnumdepth}{3}
\makeatletter
\renewcommand\paragraph[1]{\textbf{#1}\ }
\renewcommand{\theparagraph}{} %
\makeatother

\usepackage{etoolbox}
\patchcmd{\thebibliography}{\chapter*}{\section*}{}{}


==> content/open.tex <==

\section{Conclusion and Open Problems}\label{sec:conclusion}
\noindent In this work, we initiated the study of \sdom from a parameterized perspective when parameterized by solution size. 
We believe that the kernel size could still be improved.
On the other side, resolving the open complexity cases in \cref{tab:complexities} would be a natural direction for further research.
We believe the most interesting one is the parameterized complexity of \dom and \sdom on chordal bipartite graphs, as \tdom is polynomial-time solvable.
\lr{Lastly, it would be interesting to see whether \sdom is FPT for $3$-claw-free graphs.}



